Self-Triggered Output-Feedback Control of LTI Systems Subject to Disturbances and Noise

Self-triggered control (STC) and periodic event-triggered control (PETC) are aperiodic sampling techniques aiming at reducing control data communication when compared to periodic sampling. In both techniques, the effects of measurement noise in continuous-time systems with output feedback are unaddressed. In this work we prove that additive noise does not hinder stability of output-feedback PETC of linear time-invariant (LTI) systems. Then we build an STC strategy that estimates PETC's worst-case triggering times. To accomplish this, we use set-based methods, more specifically ellipsoidal sets, which describe uncertainties on state, disturbances and noise. Ellipsoidal reachability is then used to predict worst-case triggering condition violations, ultimately determining the next communication time. The ellipsoidal state estimate is recursively updated using guaranteed state estimation (GSE) methods. The proposed STC is designed to be computationally tractable at the expense of some added conservatism. It is expected to be a practical STC implementation for a broad range of applications.

==> notation.tex <==
%% Operators
\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}\!}  % (DIN) EN ISO 80000-2:2013 for transpose
\newcommand*{\traninv}{^{-{\mkern-1.5mu\mathsf{T}}}\!}  % (DIN) EN ISO 80000-2:2013 for transpose
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\dom}{dom}
% The differential operator.
\def\d{\ensuremath{\mathrm{d}}}
% Reachable operator
\DeclareMathOperator{\reach}{reach}
\def\norm[#1]{\left|#1\right|}
\def\shortnorm[#1]{|#1|}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%% Subscripts
\def\plant{{\mathrm{p}}}
\def\controller{{\mathrm{c}}}
\def\trigger{{\mathrm{t}}}
\def\controlinput{{\mathrm{u}}}
\def\disturbance{{\mathrm{w}}}
\def\noise{{\mathrm{v}}}
\def\l{{\mathrm{l}}}
\def\output{{\mathrm{y}}}

%% Sets
% (System)
\def\Xs{\mathcal{X}}
\def\Ys{\mathcal{Y}}
\def\Us{\mathcal{U}}
\def\Ws{\mathcal{W}}
\def\Vs{\mathcal{V}}
% (Outer-approximation)
\def\Ustilde{\tilde{\Us}}
\def\Wstilde{\tilde{\Ws}}
\def\Vstilde{\tilde{\Vs}}
% (Standard)
\def\No{\mathbb{N}_{0}}
\def\N{\mathbb{N}}
\def\R{\mathbb{R}}
\def\S{\mathbb{S}}
% (Function spaces)
\def\Ltwo{\mathcal{L}_2}
\def\Linf{\mathcal{L}_{\infty}}
% (Function sets)
\def\Fsu{\mathcal{F}_{\Us}}
\def\Fsw{\mathcal{F}_{\Ws}}
% (Collections for sub-indices)
\def\Ns{\mathcal{N}}
\def\Is{\mathcal{I}}
\def\Js{\mathcal{J}}
% (State-space partions)
\def\Rs{\mathcal{R}}
\def\Ss{\mathcal{S}}
% (Ellipsoid)
\def\Es{\mathcal{E}}
\def\Ks{\mathcal{C}}
\def\Bs{\mathcal{B}}
% State estimation
\def\Xstilde{\tilde{\Xs}}
\def\Xsy{\Xs_\output}
% Disturbance reachability
\def\Xw{\Xs_\disturbance}
\def\Xwtilde{\tilde{\Xs}_\disturbance}
\def\Ls{\mathcal{L}}
% Sampling times
\def\Ts{\mathcal{T}}
% General hybrid definitions
\def\Cs{\mathcal{C}}
\def\Ds{\mathcal{D}}

%% Sizes
\def\np{{n_\plant}}
\def\nup{{n_{\mathrm{u}}}}
%\def\nx{{n_{\mathrm{x}}}}
\def\ny{{n_{\mathrm{y}}}}
\def\nw{{n_{\mathrm{w}}}}
\def\nv{{n_{\mathrm{v}}}}
\def\nd{{n_{\mathrm{d}}}}
\def\nc{{n_\controller}}
\def\nt{{n_\trigger}}
\def\nl{{n_\l}}
\def\nH{{n_\mathrm{H}}}

%% Vectors
% (Points in space)
\def\xv{\boldsymbol{x}}
\def\yv{\boldsymbol{y}}
\def\uv{\boldsymbol{u}}
\def\wv{\boldsymbol{w}}
\def\vv{\boldsymbol{v}}
% (Corresponding trajectories)
\def\xiv{\boldsymbol{\xi}}
\def\upsilonv{\boldsymbol{\upsilon}}
\def\psiv{\boldsymbol{\psi}}
\def\omegav{\boldsymbol{\omega}}
\def\nuv{\boldsymbol{\nu}}
\def\zetav{\boldsymbol{\zeta}}
\def\deltav{\boldsymbol{\delta}}
\def\xixuw{\xiv_{\xp\hat{\upsilonv}\omegav}}
\def\chiv{\boldsymbol{\chi}}
% (Auxiliary)
\def\thetav{\boldsymbol{\theta}}
\def\dv{\boldsymbol{d}}
\def\sv{\boldsymbol{s}}
\def\cv{\boldsymbol{c}}
\def\qv{\boldsymbol{q}}
% (Other vector-valued functions)
\def\fv{\boldsymbol{f}}
\def\gv{\boldsymbol{g}}
\def\hv{\boldsymbol{h}}
% (For elliposoid definition)
\def\mv{\boldsymbol{m}}
\def\lv{\boldsymbol{l}}
\def\ev{\boldsymbol{e}}
\def\bv{\boldsymbol{b}}
% (Plant and controller)
\def\xip{\xiv_\plant}
\def\xic{\xiv_\controller}
\def\xc{\xv_\controller}
\def\xp{\xv_\plant}
\def\fc{\fv_\controller}
\def\gc{\gv_\controller}
% (Vector-valued triggering condition)
\def\etav{\boldsymbol{\eta}}
% (For the problem formulation)
\def\zv{\boldsymbol{z}}
\def\pv{\boldsymbol{p}}
% Estimates
\def\xptilde{\tilde{\xv}_\plant}
\def\xiptilde{\tilde{\xiv}_\plant}
\def\ytilde{\tilde{\yv}}
\def\ptilde{\tilde{\pv}}

%% Matrices 
% (System)
\def\Am{\boldsymbol{A}}
\def\Bm{\boldsymbol{B}}
\def\Cm{\boldsymbol{C}}
\def\Dm{\boldsymbol{D}}
\def\Em{\boldsymbol{E}}
% (SF Controller)
\def\Km{\boldsymbol{K}}
% (Constant matrices)
\def\I{\mathbf{I}}
\def\O{\mathbf{0}}
% (Auxiliary)
\def\Fm{\boldsymbol{F}}
\def\Gm{\boldsymbol{G}}
\def\Hm{\boldsymbol{H}}
\def\Jm{\boldsymbol{J}}
% (Transition matrices)
\def\Mm{\boldsymbol{M}}
\def\Nm{\boldsymbol{N}}
\def\CE{\Cm_{\mathrm{E}}}
\def\DE{\Dm_{\mathrm{E}}}
% (Lyapunov)
\def\Pm{\boldsymbol{P}}
% (Triggering)
\def\Qm{\boldsymbol{Q}}
\def\Qbar{\bar{\Qm}}
% (More auxiliary)
\def\Rm{\boldsymbol{R}}
\def\Sm{\boldsymbol{S}}
\def\Um{\boldsymbol{U}}
% (Set-values shape matrices)
\def\Xm{\boldsymbol{X}}
\def\Ym{\boldsymbol{Y}}
\def\Wm{\boldsymbol{W}}
\def\Vm{\boldsymbol{V}}
\def\Zm{\boldsymbol{Z}}
% (Linear plant and controller)
\def\Ap{\Am_\plant}
\def\Bp{\Bm_\plant}
\def\Cp{\Cm_\plant}
\def\Ac{\Am_\controller}
\def\Bc{\Bm_\controller}
\def\Cc{\Cm_\controller}
\def\Dc{\Dm_\controller}
% Discrete formulations
\def\Gammam{\matrixsym{\Gamma}}
\def\Phim{\matrixsym{\Phi}}
\def\Gammac{\Gammam_\controller}
\def\Gammap{\Gammam_\plant}
\def\Phic{\Phim_\controller}
\def\Phip{\Phim_\plant}
% Parameter for reachability
\def\Lm{\boldsymbol{L}}
% Observability matrix
\def\Om{\boldsymbol{O}}

%% Scalars
%\def\dk{{\Delta k}}
\def\dk{{\kappa}}
\def\LC{L_\mathrm{C}}
\def\LD{L_\mathrm{D}}

%% Others
\def\IO{\begin{bmatrix} \I & \O \end{bmatrix}}
\def\OI{\begin{bmatrix} \O & \I \end{bmatrix}}
\def\xix{\xv}  % was \xi_x
\def\thk{\thetav_{\!\dk}}
\def\Mk{\Mm_{\dk}}
\def\Nk{\Nm_{\dk}}
\def\Qk{\Qm_{\dk}}
\def\MkCE{\begin{bmatrix} \Mk \\ \CE \end{bmatrix}}
\def\NkCE{\begin{bmatrix}\Nk \\ \CE\end{bmatrix}}
\def\NkCEt{\begin{bmatrix}\Nk\tran & \CE\tran\,\end{bmatrix}}
\def\Qot{\begin{bmatrix}\bar{\Qm}_1 \\ \bar{\Qm}_2\tran\end{bmatrix}}
\def\Cth{\begin{bmatrix} \I \\ \O \end{bmatrix}}
\def\Thk{\Theta_{\Delta k}}
\def\Qott{\begin{bmatrix}\bar{\Qm}_1 & \bar{\Qm}_2\end{bmatrix}}
\def\yb{\bar{\yv}}
\def\yc{\yb_0}
\def\dy{\dv_{\yb}}
\def\Qkj{\Qk|_{\bullet, \Js}}
\def\Qkjj{\Qk|_{\Js\!, \Js}}
\def\Qkjn{\Qk|_{\Js\!, \Ns}}
\def\xt{\tilde{\xv}}
\def\Mkj{\Mm_{\dk}|_{\Js\!,\bar{\Js}}}
\def\Mkjj{\Mm_{\dk}|_{\Js\!,\Js}}
\def\Nk{\Nm_{\dk}}
\def\maxeig{\lambda_{\max}}
\def\tmiet{\tau_{\mathrm{miet}}}
\def\tmax{\bar{\tau}}

%% Lp stability stuff
\def\kyf{k_\mathrm{yf}}
\def\kyg{k_\mathrm{yg}}
\def\kdf{k_\mathrm{df}}
\def\kdg{k_\mathrm{dg}}

%% Mathematical constants
\def\e{\mathrm{e}}
\def\piconst{\text{\pi}}

%% Auxiliary matrices for Theorem
\def\Fw{\Fm_\disturbance}
\def\Fv{\Fm_\noise}
\def\Rw{\Rm_\disturbance}
\def\Rv{\Rm_\noise}
\def\Qw{\Qm_\disturbance}
\def\Qv{\Qm_\noise}
\def\cvw{c_{\noise\disturbance}}
\def\cvv{c_{\noise}}
\def\Cw{\Cm_\disturbance}
\def\Cv{\Cm_\noise}

==> with_noise_data.tex <==
\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
0	20\\
0.01	17.24312384695\\
0.01	17.24312384695\\
0.03	13.3528002608251\\
0.05	11.2952828487594\\
0.07	10.2871267235707\\
0.09	9.7991988555055\\
0.1	9.64093041067376\\
0.11	9.51453429158763\\
0.13	9.33338097428808\\
0.15	9.18141855501777\\
0.19	8.92468110553691\\
0.24	8.54511159105368\\
0.3	8.05538976818728\\
0.36	7.56321656590144\\
0.43	7.01322926511148\\
0.51	6.42983164527117\\
0.6	5.8366995256337\\
0.7	5.26164410519758\\
0.82	4.6656280810087\\
0.97	4.10506575420869\\
1.11	3.6744272613548\\
1.2	3.46130337216875\\
1.29	3.23047212783514\\
1.35	3.11222831817249\\
1.42	2.95425283925986\\
1.48	2.83379212496044\\
1.54	2.71715104999416\\
1.6	2.6033487473803\\
1.65	2.51020641657669\\
1.7	2.42200539803678\\
1.75	2.33696743382194\\
1.8	2.24943069802702\\
1.85	2.16101600132846\\
1.9	2.08071731465445\\
1.94	2.01565339869775\\
1.98	1.95419335385468\\
2.03	1.87981679713525\\
2.06	1.83850917729809\\
2.1	1.78189817778244\\
2.14	1.72143254744538\\
2.17	1.68411445744634\\
2.21	1.62585703668673\\
2.23	1.60017723331716\\
2.25	1.57390378400491\\
2.28	1.53350562654822\\
2.31	1.49522259981442\\
2.33	1.47057624017675\\
2.36	1.43075587012824\\
2.38	1.406814109255\\
2.4	1.38251928051074\\
2.43	1.34353303492969\\
2.45	1.31827229486611\\
2.46	1.30767585063269\\
2.48	1.28305001346618\\
2.49	1.27216474642902\\
2.5	1.26042007764436\\
2.51	1.25029235700201\\
2.52	1.2389341318481\\
2.53	1.22801402680164\\
2.54	1.21663689700057\\
2.55	1.20717263430037\\
2.56	1.19570635560151\\
2.57	1.18559950974322\\
2.58	1.17408431612127\\
2.59	1.16463271816035\\
2.6	1.15447606401958\\
2.61	1.14360624077621\\
2.62	1.13320532296176\\
2.63	1.12379193910577\\
2.64	1.11385931948466\\
2.65	1.10439474823056\\
2.66	1.092933541322\\
2.67	1.08373866725716\\
2.68	1.07312590676005\\
2.69	1.06348831574746\\
2.7	1.05429554569735\\
2.71	1.04450103226791\\
2.72	1.03524886368179\\
2.73	1.02462265318921\\
2.74	1.01547924932061\\
2.75	1.00606468845858\\
2.76	0.996749797692038\\
2.77	0.986455886510774\\
2.78	0.976766258870747\\
2.79	0.967064068830471\\
2.8	0.957809604851775\\
2.81	0.94872110312881\\
2.82	0.93946103865208\\
2.83	0.930149308949397\\
2.84	0.920321410963628\\
2.85	0.911693947027638\\
2.86	0.902794822419858\\
2.87	0.894539389431369\\
2.88	0.885351584587011\\
2.89	0.876388903722439\\
2.9	0.867477600058097\\
2.91	0.859958381110316\\
2.92	0.850969030875281\\
2.93	0.84347560235472\\
2.94	0.835587192687997\\
2.95	0.827668007069272\\
2.96	0.819724112526099\\
2.97	0.812684484444434\\
2.98	0.804421648776436\\
2.99	0.796672846362018\\
3	0.78855058459223\\
3.01	0.780057120648407\\
3.02	0.771903583565158\\
3.03	0.764935985792328\\
3.04	0.758146965089082\\
3.05	0.75022118204544\\
3.06	0.742781848906034\\
3.07	0.73536502349881\\
3.08	0.72791369898678\\
3.09	0.721199314969623\\
3.1	0.714329366080889\\
3.11	0.706660870561546\\
3.12	0.699830703795296\\
3.13	0.693062193479674\\
3.14	0.685701729848548\\
3.15	0.678338890508334\\
3.16	0.670865774405401\\
3.17	0.664963298895133\\
3.18	0.657899259149961\\
3.19	0.651811270572591\\
3.2	0.644760755729668\\
3.21	0.637667556833398\\
3.22	0.631113100195523\\
3.23	0.624393989779502\\
3.24	0.618111767617174\\
3.25	0.611325171085294\\
3.26	0.605945456259465\\
3.27	0.598856047988241\\
3.28	0.591807304308391\\
3.29	0.585008780759056\\
3.3	0.579025333489736\\
3.31	0.573757682350726\\
3.32	0.568055201292992\\
3.33	0.562272264337377\\
3.34	0.556580908639347\\
3.35	0.549457667072947\\
3.36	0.543668347566011\\
3.37	0.537490499979921\\
3.38	0.530314279030001\\
3.39	0.524202389860726\\
3.4	0.518413299013871\\
3.41	0.51215891208874\\
3.42	0.506554351014889\\
3.43	0.501014349318113\\
3.44	0.494464586925371\\
3.45	0.488621421364928\\
3.46	0.482921771862246\\
3.47	0.477266988295517\\
3.48	0.47245472202028\\
3.49	0.46681837173038\\
3.5	0.461228821433542\\
3.51	0.456570700015264\\
3.52	0.451316975048548\\
3.53	0.446585918966822\\
3.54	0.441488604571926\\
3.55	0.437037100426247\\
3.56	0.431743085412544\\
3.57	0.426911432318346\\
3.58	0.421896170222482\\
3.59	0.417709741493033\\
3.6	0.412511533982393\\
3.61	0.407618697124067\\
3.62	0.402532190623555\\
3.63	0.397724787054944\\
3.64	0.393283772380848\\
3.65	0.388098499230283\\
3.66	0.384609222498703\\
3.67	0.379489338988281\\
3.68	0.375352435533057\\
3.69	0.371168596883869\\
3.7	0.366853447265499\\
3.71	0.36323534661029\\
3.72	0.358693441119951\\
3.73	0.355676965307646\\
3.74	0.351788718931447\\
3.75	0.347786274394997\\
3.76	0.343209346510624\\
3.77	0.339211983543517\\
3.78	0.334887710152611\\
3.79	0.330213799524564\\
3.8	0.326814477632297\\
3.81	0.322162536081877\\
3.82	0.318794567704993\\
3.83	0.315251676599553\\
3.84	0.31111436573236\\
3.85	0.307426504382282\\
3.86	0.303306892633681\\
3.87	0.299406539034402\\
3.88	0.295601680167373\\
3.89	0.292810990251105\\
3.9	0.288350852693004\\
3.91	0.284622660056179\\
3.92	0.280385964150691\\
3.93	0.276573037199629\\
3.94	0.272745413369795\\
3.95	0.270461159104\\
3.96	0.266343620238555\\
3.97	0.262665262973937\\
3.98	0.259704547904852\\
3.99	0.256041771124239\\
4	0.252398394840519\\
4.01	0.249533397788547\\
4.02	0.246831880240372\\
4.03	0.242990781388855\\
4.04	0.239450395140772\\
4.05	0.237194611570741\\
4.06	0.234471680822592\\
4.07	0.231616975765467\\
4.08	0.228839364964293\\
4.09	0.226640714137566\\
4.1	0.224181117742414\\
4.11	0.21991066896532\\
4.12	0.216760644669924\\
4.13	0.213704279738315\\
4.14	0.21010729700445\\
4.15	0.207787845386465\\
4.16	0.204135094528583\\
4.17	0.20106052013422\\
4.18	0.198463296129803\\
4.19	0.195702726915328\\
4.2	0.193369469204287\\
4.21	0.191052221668211\\
4.22	0.189078842806012\\
4.23	0.186538239942632\\
4.24	0.183424650872987\\
4.25	0.180553245748283\\
4.26	0.177918299180178\\
4.27	0.17603276974252\\
4.28	0.173656391439403\\
4.29	0.171176828204977\\
4.3	0.168574073926322\\
4.31	0.165352677944224\\
4.32	0.162308835821868\\
4.33	0.160042677494046\\
4.34	0.158432004497189\\
4.35	0.155177124419753\\
4.36	0.153009093702152\\
4.37	0.151556989578195\\
4.38	0.148477830713339\\
4.39	0.145828649867444\\
4.4	0.14323697868243\\
4.41	0.141990646182099\\
4.42	0.140668523470555\\
4.43	0.139060300355115\\
4.44	0.137360831720449\\
4.45	0.13553314552743\\
4.46	0.133719165974969\\
4.47	0.130574664472199\\
4.48	0.128458483392164\\
4.49	0.12652695084867\\
4.5	0.123460701292782\\
4.51	0.12056782043892\\
4.52	0.11887378517414\\
4.53	0.1166342921346\\
4.54	0.115090167267571\\
4.55	0.112978468588693\\
4.56	0.110333426838559\\
4.57	0.107880223119856\\
4.58	0.106368805535712\\
4.59	0.104545108202928\\
4.6	0.103200199976337\\
4.61	0.101285298882258\\
4.62	0.100051980539223\\
4.63	0.0982055698052872\\
4.64	0.0960883436658796\\
4.65	0.0948213636447034\\
4.66	0.0925764328450863\\
4.67	0.0909073892753603\\
4.68	0.0889027913578752\\
4.69	0.0872603733070191\\
4.7	0.0853534576180176\\
4.71	0.0834948352544432\\
4.72	0.081534981936257\\
4.73	0.0802383210351607\\
4.74	0.0785334873521517\\
4.75	0.0768273670848112\\
4.76	0.0757150146947862\\
4.77	0.0740176829271214\\
4.78	0.07243358295513\\
4.79	0.0709606313354964\\
4.8	0.0695804943257504\\
4.81	0.0685491844658746\\
4.82	0.0679132654236878\\
4.83	0.0662671155318863\\
4.84	0.0651920436242856\\
4.85	0.0637995564666046\\
4.86	0.0623651737411133\\
4.87	0.0619053902699683\\
4.88	0.0608878720069077\\
4.89	0.0594582805021502\\
4.9	0.0581288785167984\\
4.91	0.0570700765140856\\
4.92	0.0568216099202896\\
4.93	0.0563314696171229\\
4.94	0.0557478870812241\\
4.95	0.0544544007463104\\
4.96	0.0528367329447678\\
4.97	0.0519740447625376\\
4.98	0.0502152167504459\\
4.99	0.0488818944916999\\
5	0.0482222391853755\\
5.01	0.0469278985829219\\
5.02	0.0458223840810491\\
5.03	0.0448054085560518\\
5.04	0.0437207424846435\\
5.05	0.0432489576378017\\
5.06	0.0426280246229668\\
5.07	0.0413485153907553\\
5.08	0.0401173890264932\\
5.09	0.039226587831842\\
5.1	0.0385465098022059\\
5.11	0.0372250611982712\\
5.12	0.0364741081244251\\
5.13	0.0360238155035649\\
5.14	0.0358365535758397\\
5.15	0.0353026103729259\\
5.16	0.0342622589152064\\
5.17	0.033499160758936\\
5.18	0.0328974704902696\\
5.19	0.0320383909896021\\
5.2	0.0320010593398488\\
5.21	0.031309736245501\\
5.22	0.0312800100086013\\
5.23	0.0306853607657519\\
5.24	0.0302082186686829\\
5.25	0.0296972227716364\\
5.26	0.029341175737553\\
5.27	0.0293368444744243\\
5.28	0.0294195950495213\\
5.29	0.0291831989772991\\
5.3	0.028240412173187\\
5.31	0.027476701463039\\
5.32	0.0268126523045315\\
5.33	0.0269794961075805\\
5.34	0.0272330914565645\\
5.35	0.0267323644133748\\
5.36	0.0260705332132478\\
5.37	0.0258620977136285\\
5.38	0.0257479269030506\\
5.39	0.0251557057925276\\
5.4	0.0245712618955473\\
5.41	0.025235038075277\\
5.42	0.0253474663223725\\
5.43	0.0254143901445641\\
5.44	0.0255017556552622\\
5.45	0.0251270420814713\\
5.46	0.0250161485211493\\
5.47	0.02360779230215\\
5.48	0.0232421211826507\\
5.49	0.0223196187625091\\
5.5	0.0217299206286351\\
5.51	0.0220898953419205\\
5.52	0.0209816116522677\\
5.53	0.0208649310724267\\
5.54	0.0200101939857566\\
5.55	0.0193369989420419\\
5.56	0.0196219647522764\\
5.57	0.0191662189847117\\
5.58	0.0186945916277805\\
5.59	0.0187463718698211\\
5.6	0.0185395443114556\\
5.61	0.0183303053665316\\
5.62	0.0185934600323137\\
5.63	0.0184568970948894\\
5.64	0.0190335009044748\\
5.65	0.0189441594308775\\
5.66	0.0187598475400139\\
5.67	0.0185994280893557\\
5.68	0.0184298247256289\\
5.69	0.0181310157397922\\
5.7	0.0180758908542772\\
5.71	0.0183198951326099\\
5.72	0.0185882254292357\\
5.73	0.0182119716462215\\
5.74	0.0177757727223515\\
5.75	0.0176449320012171\\
5.76	0.0170106443318837\\
5.77	0.0172597138970094\\
5.78	0.0174309227088091\\
5.79	0.0169923326839568\\
5.8	0.0161576046077923\\
5.81	0.0155026893996663\\
5.82	0.0146654332960173\\
5.83	0.0149982427189646\\
5.84	0.0148878581085042\\
5.85	0.0146426795156498\\
5.86	0.0142477499136831\\
5.87	0.0140058846381479\\
5.88	0.0132423883444099\\
5.89	0.0129098842846159\\
5.9	0.0133628116262705\\
5.91	0.0127947510521259\\
5.92	0.0129335796568481\\
5.93	0.0130707832141173\\
5.94	0.0126222871798707\\
5.95	0.0125438349861744\\
5.96	0.0130237614468936\\
5.97	0.0121231818137862\\
5.98	0.0119502302601166\\
5.99	0.0119957407566986\\
6	0.0116264602939096\\
6.01	0.0119056412942697\\
6.02	0.0118212071071017\\
6.03	0.0110075571348796\\
6.04	0.0109199798805447\\
6.05	0.010910125005758\\
6.06	0.0105225155106421\\
6.07	0.0106192856196039\\
6.08	0.0105965040972168\\
6.09	0.0112389185001717\\
6.1	0.0108843669741896\\
6.11	0.0111514522909465\\
6.12	0.010865632118394\\
6.13	0.0106049507523052\\
6.14	0.0104148628259673\\
6.15	0.0105911581049691\\
6.16	0.0103364199476694\\
6.17	0.0101797870434132\\
6.18	0.0101688157995369\\
6.19	0.010235376066697\\
6.2	0.0103331391797604\\
6.21	0.0102611156240328\\
6.22	0.0102842435339065\\
6.23	0.00993825473561331\\
6.24	0.00985823197819842\\
6.25	0.0100040398803179\\
6.26	0.0100314031488681\\
6.27	0.0103107538998222\\
6.28	0.00999092365322463\\
6.29	0.00949921503984688\\
6.3	0.00946709201925527\\
6.31	0.00891501408766674\\
6.32	0.00883479189199285\\
6.33	0.00856469629724805\\
6.34	0.00812428701070045\\
6.35	0.00805237509351778\\
6.36	0.00785908701723817\\
6.37	0.00738433127808663\\
6.38	0.00740325430253233\\
6.39	0.00745117965664494\\
6.4	0.00804754878004669\\
6.41	0.00838975154871251\\
6.42	0.00806990162421859\\
6.43	0.00766543541761409\\
6.44	0.00765536246899787\\
6.45	0.00726267047229881\\
6.46	0.0072607180169763\\
6.47	0.00733073724456025\\
6.48	0.00756732875917779\\
6.49	0.0077818614784196\\
6.5	0.00796348675694984\\
6.51	0.00738074780722499\\
6.52	0.0068604155919761\\
6.53	0.00697235459182271\\
6.54	0.00659537385974309\\
6.55	0.0067665124554145\\
6.56	0.00650534273583666\\
6.57	0.00703348350997283\\
6.58	0.00696108914306047\\
6.59	0.0069282352211197\\
6.6	0.00631999809931736\\
6.61	0.00668728011850555\\
6.62	0.00668680749202191\\
6.63	0.0062849197200761\\
6.64	0.00599684033155984\\
6.65	0.00607490077113978\\
6.66	0.0062665424760938\\
6.67	0.00598648592819945\\
6.68	0.00643382824074334\\
6.69	0.00742746222168141\\
6.7	0.00706794616241862\\
6.71	0.00662837380138905\\
6.72	0.00678932716122321\\
6.73	0.00701200008522019\\
6.74	0.00642104517095953\\
6.75	0.00633929641958644\\
6.76	0.00611355703245539\\
6.77	0.00618732958216321\\
6.78	0.00612053154718697\\
6.79	0.00598936335453189\\
6.8	0.00541826869783642\\
6.81	0.00529517392881709\\
6.82	0.00504469359187987\\
6.83	0.00486463418085905\\
6.84	0.00472678269424671\\
6.85	0.00468891689011407\\
6.86	0.00445007743624332\\
6.87	0.00487833759644026\\
6.88	0.00482647619632635\\
6.89	0.00449231685528297\\
6.9	0.00479328462781304\\
6.91	0.00535014802209946\\
6.92	0.00603068492499692\\
6.93	0.00628031356199299\\
6.94	0.0066080567088724\\
6.95	0.00669126340839171\\
6.96	0.00603576908112318\\
6.97	0.00582476513214171\\
6.98	0.00598108278073027\\
6.99	0.00558459044604208\\
7	0.00478280102359896\\
7.01	0.00486329753062768\\
7.02	0.0043752465437774\\
7.03	0.00412016228708951\\
7.04	0.00403831896650716\\
7.05	0.00395548958008658\\
7.06	0.00414081941187867\\
7.07	0.00390760539095625\\
7.08	0.00424351435649803\\
7.09	0.00450630296495447\\
7.1	0.00426752255625181\\
7.11	0.00404382476674553\\
7.12	0.00457355407114682\\
7.13	0.00493699410471794\\
7.14	0.00520941313096369\\
7.15	0.0053509334784121\\
7.16	0.0046640199796104\\
7.17	0.00462582315506427\\
7.18	0.00579510905518197\\
7.19	0.00565818597568397\\
7.2	0.00494659921617336\\
7.21	0.00456282353947284\\
7.22	0.00489693071769319\\
7.23	0.00525376304809995\\
7.24	0.00603500805696816\\
7.25	0.00701560931061947\\
7.26	0.00565955148682071\\
7.27	0.00658725625230461\\
7.28	0.00779108342504822\\
7.29	0.00750028025907564\\
7.3	0.00762849909742257\\
7.31	0.00682995556933269\\
7.32	0.00629649843763744\\
7.33	0.00612265631005591\\
7.34	0.00580986994352507\\
7.35	0.0053799870121832\\
7.36	0.00511704184068081\\
7.37	0.00586836805688258\\
7.38	0.00640885198932669\\
7.39	0.00664584920037655\\
7.4	0.00575125201693939\\
7.41	0.00532168596702011\\
7.42	0.0054079482657283\\
7.43	0.00495615252191735\\
7.44	0.00581420082364508\\
7.45	0.00525804563266722\\
7.46	0.00456462828666937\\
7.47	0.00481332782090224\\
7.48	0.00561575362372448\\
7.49	0.00685886276277262\\
7.5	0.0056974227401315\\
7.51	0.00598651738879215\\
7.52	0.00555867128714443\\
7.53	0.00576483975354542\\
7.54	0.00567318451943912\\
7.55	0.00585397092389287\\
7.56	0.00544539083413436\\
7.57	0.00589930785313965\\
7.58	0.00758069236187331\\
7.59	0.00843023539708867\\
7.6	0.00852918207195159\\
7.61	0.00737078498236479\\
7.62	0.00627366470327015\\
7.63	0.00598001593589545\\
7.64	0.0060241539803553\\
7.65	0.00648686857691245\\
7.66	0.0059380351066852\\
7.67	0.00586220323784909\\
7.68	0.00660546123100695\\
7.69	0.0074983787155019\\
7.7	0.00889236980092102\\
7.71	0.00913994135182262\\
7.72	0.00937587555407768\\
7.73	0.00894901050940925\\
7.74	0.00808917902071647\\
7.75	0.00717698113206203\\
7.76	0.0074443346526722\\
7.77	0.00766544164791299\\
7.78	0.00783369905406476\\
7.79	0.00814098370461601\\
7.8	0.00763932388088779\\
7.81	0.00918685367118888\\
7.82	0.00857268299159241\\
7.83	0.00884023175719674\\
7.84	0.00898918311250733\\
7.85	0.0094451793689143\\
7.86	0.0092201929737189\\
7.87	0.00914458778224722\\
7.88	0.00843452903221638\\
7.89	0.00814241274417757\\
7.9	0.00957558752077214\\
7.91	0.00963486357525664\\
7.92	0.00895664120601404\\
7.93	0.00845091658580792\\
7.94	0.00785695404403947\\
7.95	0.00741841478569322\\
7.96	0.00712023321293209\\
7.97	0.00737812708546806\\
7.98	0.00749254825342232\\
7.99	0.00679678921458611\\
8	0.0064381160632228\\
8.01	0.00680565773764176\\
8.02	0.00755756420173536\\
8.03	0.00817966462356654\\
8.04	0.00811661789652228\\
8.05	0.00900941543015563\\
8.06	0.00821914268963398\\
8.07	0.00853310050045604\\
8.08	0.00936910729586942\\
8.09	0.00861535700693864\\
8.1	0.00882609504165333\\
8.11	0.00789343656573687\\
8.12	0.00852973227383588\\
8.13	0.0086222807976809\\
8.14	0.00758980389881745\\
8.15	0.00666506752594847\\
8.16	0.00654545453212557\\
8.17	0.00677906399908499\\
8.18	0.00661543711485642\\
8.19	0.00752072366878731\\
8.2	0.00778063192899536\\
8.21	0.00766421978849853\\
8.22	0.00892504379061783\\
8.23	0.008093763880762\\
8.24	0.00845311710078908\\
8.25	0.00866510330512385\\
8.26	0.00788369500009672\\
8.27	0.0073998948918527\\
8.28	0.00813387554360258\\
8.29	0.00757974252252861\\
8.3	0.00746424319664624\\
8.31	0.00738492281062624\\
8.32	0.00784823425306763\\
8.33	0.00797393142408742\\
8.34	0.00714944514703616\\
8.35	0.00732817145238499\\
8.36	0.00744576886464152\\
8.37	0.00766587253087352\\
8.38	0.00687499512217795\\
8.39	0.00734898496938044\\
8.4	0.00795699636014986\\
8.41	0.0070133090236554\\
8.42	0.0066022854825824\\
8.43	0.00572540859202875\\
8.44	0.0063081966361534\\
8.45	0.00624001793212374\\
8.46	0.00741811708442022\\
8.47	0.00779482168397693\\
8.48	0.00777153953308161\\
8.49	0.00704880965005944\\
8.5	0.00829979609146174\\
8.51	0.00884876919461891\\
8.52	0.00954933918743902\\
8.53	0.00870970138648041\\
8.54	0.00748549572751283\\
8.55	0.00658157101961199\\
8.56	0.0065138863826043\\
8.57	0.00566987792049175\\
8.58	0.00653412111916042\\
8.59	0.00681486041584671\\
8.6	0.00596206950662069\\
8.61	0.00623464307393293\\
8.62	0.00724755972670781\\
8.63	0.00715960304173113\\
8.64	0.00641280185371701\\
8.65	0.00584600007609488\\
8.66	0.0064750241784903\\
8.67	0.00523261337229832\\
8.68	0.0053328224643697\\
8.69	0.00519018446970404\\
8.7	0.00474666781244111\\
8.71	0.00518127662947258\\
8.72	0.00572739672210858\\
8.73	0.00585119849161457\\
8.74	0.00590770146894988\\
8.75	0.00551772277979445\\
8.76	0.0057067537706503\\
8.77	0.00532514607899206\\
8.78	0.00603555585501981\\
8.79	0.00631321155162723\\
8.8	0.00503659258904096\\
8.81	0.00463209128855368\\
8.82	0.00508092762191463\\
8.83	0.00511072305961846\\
8.84	0.00444314989467953\\
8.85	0.00411248873086114\\
8.86	0.00379743589164687\\
8.87	0.00363273344512529\\
8.88	0.00375192919215677\\
8.89	0.00335612636343993\\
8.9	0.00322692102251762\\
8.91	0.00326929604332962\\
8.92	0.00372467336678838\\
8.93	0.00409776857478793\\
8.94	0.00421928922472862\\
8.95	0.00508290228908693\\
8.96	0.00395276659194441\\
8.97	0.00364206558951846\\
8.98	0.00397379193543931\\
8.99	0.00302581673175935\\
9	0.00389361782025933\\
9.01	0.00360907152339467\\
9.02	0.00353286571352346\\
9.03	0.00364415614004147\\
9.04	0.0029758842173421\\
9.05	0.00299084365774845\\
9.06	0.00333269343367145\\
9.07	0.00305788967009002\\
9.08	0.0026058311229894\\
9.09	0.00263879004527974\\
9.1	0.00283745748220765\\
9.11	0.00250124588968442\\
9.12	0.0029323349216653\\
9.13	0.00265750000525949\\
9.14	0.0029071232001265\\
9.15	0.00267146053077854\\
9.16	0.00286658060797032\\
9.17	0.00261354890657049\\
9.18	0.00235590560459708\\
9.19	0.00221822564269497\\
9.2	0.00201920958365568\\
9.21	0.0019573356594155\\
9.22	0.00205682536870052\\
9.23	0.00233835888351443\\
9.24	0.0019327146150118\\
9.25	0.00220214923978566\\
9.26	0.00235019908256434\\
9.27	0.00272389929393104\\
9.28	0.0029934377439234\\
9.29	0.00283186462450131\\
9.3	0.00360501201885585\\
9.31	0.00328299126721528\\
9.32	0.0027360618931374\\
9.33	0.00224807304638413\\
9.34	0.00268125394222489\\
9.35	0.00236100767262159\\
9.36	0.00264697832137429\\
9.37	0.00275058204418248\\
9.38	0.00289984386910606\\
9.39	0.00277383279317841\\
9.4	0.00325958094206757\\
9.41	0.00367164495108179\\
9.42	0.00440204034215385\\
9.43	0.00451418128582486\\
9.44	0.00549141212389662\\
9.45	0.00563273496960094\\
9.46	0.00496729574033737\\
9.47	0.00513837882635705\\
9.48	0.00530592198088176\\
9.49	0.00650214137576509\\
9.5	0.00570697551793055\\
9.51	0.00623198424143138\\
9.52	0.00587100388787676\\
9.53	0.00554514792687406\\
9.54	0.00463711876458043\\
9.55	0.0034984058999244\\
9.56	0.00349144652288836\\
9.57	0.00386436611451654\\
9.58	0.00409615218211587\\
9.59	0.00460466392408717\\
9.6	0.00360948156483608\\
9.61	0.00304746978182817\\
9.62	0.00384318640169196\\
9.63	0.00375485781357235\\
9.64	0.00393901071969686\\
9.65	0.00436177039545423\\
9.66	0.00537607979842384\\
9.67	0.00424106673817575\\
9.68	0.00490248602019372\\
9.69	0.00474159628527041\\
9.7	0.0038259585755949\\
9.71	0.00332787021311678\\
9.72	0.00292399342606084\\
9.73	0.00364889039504084\\
9.74	0.00314600712210377\\
9.75	0.00284240397758868\\
9.76	0.00316316785084151\\
9.77	0.00359309350962251\\
9.78	0.00381222660669073\\
9.79	0.00367093768706533\\
9.8	0.00348379770132819\\
9.81	0.00484232791416783\\
9.82	0.0037720046801452\\
9.83	0.00296585985162787\\
9.84	0.00295053914203176\\
9.85	0.00399741003833376\\
9.86	0.00440613321527996\\
9.87	0.0053656920524827\\
9.88	0.00561856386976853\\
9.89	0.00566090873911098\\
9.9	0.00491042258318545\\
9.91	0.00452819825835935\\
9.92	0.00460109278960388\\
9.93	0.00439385945583581\\
9.94	0.00471297000573687\\
9.95	0.00536640368919574\\
9.96	0.00647649022869207\\
9.97	0.00525872490560096\\
9.98	0.00412314355021326\\
9.99	0.00389810819983937\\
10	0.00410048825808619\\
};
\addlegendentry{PSTC $\epsilon=0$}

\addplot [color=mycolor2, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	20\\
0.01	17.24312384695\\
0.01	17.24312384695\\
0.03	13.3528002608251\\
0.05	11.2952828487594\\
0.07	10.2871267235707\\
0.09	9.7991988555055\\
0.1	9.64093041067376\\
0.11	9.51453429158763\\
0.13	9.33338097428808\\
0.15	9.18141855501777\\
0.19	8.92468110553691\\
0.25	8.47713704970525\\
0.31	7.9831080458001\\
0.38	7.40559956637681\\
0.45	6.87342522773469\\
0.53	6.30057857015152\\
0.62	5.71953768965533\\
0.73	5.10925996987364\\
0.86	4.5168053097883\\
1.02	3.93821066906395\\
1.16	3.56699612373155\\
1.27	3.27652079127435\\
1.36	3.0917647911987\\
1.45	2.90415337407913\\
1.53	2.74178106910511\\
1.6	2.61298985292438\\
1.68	2.45608760889134\\
1.76	2.30879711103845\\
1.83	2.20054403813949\\
1.92	2.04078719490023\\
1.99	1.94083254140712\\
2.08	1.79670680552983\\
2.18	1.65547588208762\\
2.27	1.53024685140365\\
2.35	1.4318876304185\\
2.46	1.29433297188641\\
2.57	1.16553609633483\\
2.69	1.04468935661077\\
2.79	0.963726914726376\\
2.9	0.850148911963502\\
3	0.78195506721445\\
3.11	0.681206048264544\\
3.19	0.641401223608293\\
3.31	0.548316649510742\\
3.43	0.489718618752139\\
3.54	0.404101676018806\\
3.65	0.37758312150049\\
3.77	0.323774266666085\\
3.89	0.275809081777039\\
4.02	0.230434209051979\\
4.17	0.183488297131748\\
4.32	0.153699223517397\\
4.45	0.125004182048937\\
4.58	0.109175502013073\\
4.68	0.0796226734208097\\
4.83	0.0653600382784762\\
4.95	0.0515114610032624\\
5.09	0.0358077479473079\\
5.21	0.0227681197298878\\
5.36	0.0166406050623618\\
5.51	0.01610894257375\\
5.66	0.0285762103639753\\
5.78	0.0245157974745712\\
5.93	0.0118908954268975\\
6.08	0.0211301772768837\\
6.22	0.0230088190059345\\
6.37	0.0176646484867856\\
6.52	0.0213708480660672\\
6.67	0.0177214939353183\\
6.82	0.0195563026184918\\
6.95	0.0181507987609738\\
7.1	0.00661957443349758\\
7.25	0.0141217941678256\\
7.4	0.0177855868973842\\
7.55	0.0142782647844216\\
7.7	0.0196731594039024\\
7.81	0.0254764102622898\\
7.93	0.0178790671783866\\
8.05	0.0133175361143127\\
8.2	0.0160929264248648\\
8.33	0.014250536652831\\
8.45	0.0170763161899588\\
8.56	0.030244324879644\\
8.65	0.0151719847811957\\
8.75	0.0184179660712143\\
8.87	0.0116287997567921\\
9.02	0.00778363836330843\\
9.17	0.015417830559414\\
9.32	0.0068502879740784\\
9.46	0.0257072120477266\\
9.58	0.0145610866765813\\
9.7	0.0269456417443352\\
9.82	0.0171623335179007\\
9.96	0.0063345348650204\\
};
\addlegendentry{PSTC $\epsilon = 0.1$}
